Certainty In, Certainty Out: REVQCs for Quantum Machine Learning

The field of Quantum Machine Learning (QML) has emerged recently in the hopes of finding new machine learning protocols or exponential speedups for classical ones. Apart from problems with vanishing gradients and efficient encoding methods, these speedups are hard to find because the sampling nature of quantum computers promotes either simulating computations classically or running them many times on quantum computers in order to use approximate expectation values in gradient calculations. In this paper, we make a case for setting high single-sample accuracy as a primary goal. We discuss the statistical theory which enables highly accurate and precise sample inference, and propose a method of reversed training towards this end. We show the effectiveness of this training method by assessing several effective variational quantum circuits (VQCs), trained in both the standard and reversed directions, on random binary subsets of the MNIST and MNIST Fashion datasets, on which our method provides an increase of $10-15\%$ in single-sample inference accuracy.

==> circfigs.tex <==

\begin{figure}
    \begin{subfigure}[h]{.35\textwidth}
        \begin{subfigure}{\textwidth}
          \centering
          \includegraphics[width=.8\linewidth]{figs/circs/circ.pdf}
          \caption{Full circuit}
          \label{fig:circ}
        \end{subfigure}
    \end{subfigure}
    \begin{subfigure}[h]{.35\textwidth}
        \begin{subfigure}{.47\textwidth}
          \centering
          \includegraphics[width=\linewidth]{figs/circs/cnn6.pdf}
          \caption{CNN6}
          \label{fig:cnn6}
        \end{subfigure}%
        \begin{subfigure}{.47\textwidth}
          \centering
          \includegraphics[width=\linewidth]{figs/circs/cnn7.pdf}
          \caption{CNN7}
          \label{fig:cnn7}
        \end{subfigure}
         \\
        \begin{subfigure}{.47\textwidth}
          \centering
          \includegraphics[width=\linewidth]{figs/circs/cnn8.pdf}
          \caption{CNN8}
          \label{fig:cnn8}
        \end{subfigure}
        \begin{subfigure}{.47\textwidth}
          \centering
          \includegraphics[width=\linewidth]{figs/circs/cnn9.pdf}
          \caption{CNN9}
          \label{fig:cnn9}
        \end{subfigure}
    \end{subfigure} 
    \begin{subfigure}[h]{.28\textwidth}
        \begin{subfigure}{.8\textwidth}
          \centering
          \includegraphics[width=\linewidth]{figs/circs/pool.pdf}
          \caption{Pooling}
          \label{fig:pool}
        \end{subfigure}
    \end{subfigure}
\caption{Unitary circuits used in the QCNN.}
\label{fig:circuits}
\end{figure}


%\begin{figure}
%\subfloat[fig 1]{\includegraphics[width = 3in]{something}} 
%\subfloat[fig 2]{\includegraphics[width = 3in]{something}}\\
%\subfloat[fig 3]{\includegraphics[width = 3in]{something}}
%\subfloat[fig 4]{\includegraphics[width = 3in]{something}} 
%\caption{Add your own figures before compiling}
%\label{some example}
%\end{figure}
